Pulsating Components in Binary and Multiple Stellar Systems --- A Catalog of Oscillating Binaries

We present an up-to-date catalog of pulsating binaries, i.e. the binary and multiple stellar systems containing pulsating components, along with a statistics on them. Compared to the earlier compilation by Soydugan et al.(2006a) of 25 delta Scuti-type `oscillating Algol-type eclipsing binaries' (oEA), the recent collection of 74 oEA by Liakos et al.(2012), and the collection of Cepheids in binaries by Szabados (2003a), the numbers and types of pulsating variables in binaries are now extended. The total numbers of pulsating binary/multiple stellar systems have increased to be 515 as of 2014 October 26, among which 262+ are oscillating eclipsing binaries and the oEA containing delta Scuti components are updated to be 96. The catalog is intended to be a collection of various pulsating binary stars across the Hertzsprung-Russell diagram. We reviewed the open questions, advances and prospects connecting pulsation/oscillation and binarity. The observational implication of binary systems with pulsating components, to stellar evolution theories is also addressed. In addition, we have searched the Simbad database for candidate pulsating binaries. As a result, 322 candidates were extracted. Furthermore, a brief statistics on Algol-type eclipsing binaries (EA) based on the existing catalogs is given. We got 5315 EA, of which there are 904 EA with spectral types A and F. The present catalog has a sortable web version allowing easy updating and maintenance at http://www.chjaa.org/COB/ .

==> hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump


